A theory-based AI automation exposure index: Applying Moravec's Paradox to the US labor market

This paper develops a theory-driven automation exposure index based on Moravec's Paradox. Scoring 19,000 O*NET tasks on performance variance, tacit knowledge, data abundance, and algorithmic gaps reveals that management, STEM, and sciences occupations show the highest exposure. In contrast, maintenance, agriculture, and construction show the lowest. The positive relationship between wages and exposure challenges the notion of skill-biased technological change if AI substitutes for workers. At the same time, tacit knowledge exhibits a positive relationship with wages consistent with seniority-biased technological change. This index identifies fundamental automatability rather than current capabilities, while also validating the AI annotation method pioneered by Eloundou et al. (2024) with a correlation of 0.72. The non-positive relationship with pre-LLM indices suggests a paradigm shift in automation patterns.

==> graphics/cs_OV.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Di, Jan 16, 2024 - 11:16:13
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 1,585.459$^{***}$ \\ 
  & (21.400) \\ 
  & \\ 
 n5\_9 & 20.231$^{***}$ \\ 
  & (0.075) \\ 
  & \\ 
 n500\_999 & 598.179$^{***}$ \\ 
  & (2.246) \\ 
  & \\ 
 n1000 & 2,710.804$^{***}$ \\ 
  & (2.334) \\ 

\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 

==> graphics/cs_combined.tex <==
\begin{table}[h]
\centering
\caption{Combined Results of Specifications}
\label{tab:combined_results}
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: Employment}} \\ 
\cline{2-4} 
\\[-1.8ex] & Heterogeneity with NAs& Heterogeneity with  0s & Omitted Variable with 0s \\ 
\hline \\[-1.8ex] 
interaction\_term & 710.699$^{***}$ & 65.986$^{***}$ & 72.763$^{***}$  \\ 
 & (21.318) & (0.877) & (0.889) \\ 
 & & & \\
n5\_9 & 19.282$^{***}$ & 15.472$^{***}$ & 15.799$^{***}$\\ 
 & (0.074) & (0.048) & ( 0.048) \\ 
 & & & \\
n500\_999 & 535.465$^{***}$ & 509.666$^{***}$ & 544.907$^{***}$ \\ 
 & (2.212) & (1.637) & (1.651) \\ 
 & & & \\
n1000 & 2,276.305$^{***}$ & 2,001.274$^{***}$ & 2,658.739$^{***}$ \\ 
 & (3.142) & (3.366) & (1.656) \\ 
 & & & \\
AIGE:n1000 & 92.186$^{***}$ & 104.236$^{***}$ &  \\ 
 & (0.460) & (0.467) &  \\
\hline 
\hline \\[-1.8ex] \\ 
\end{tabular} 
\end{table}

==> graphics/cs_emp.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Do, Jan 11, 2024 - 17:28:12
\begin{table}[h] \centering 
  \caption{} 
  \label{} 

\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & Employment \\ 
\hline \\[-1.8ex] 
 interaction\_term & 710.699$^{***}$ \\ 
  & (21.318) \\ 

  & \\ 
 n5\_9 & 19.282$^{***}$ \\ 
  & (0.074) \\ 
  & \\ 
 n500\_999 & 535.465$^{***}$ \\ 
  & (2.212) \\ 
  & \\ 
 n1000 & 2,276.305$^{***}$ \\ 
  & (3.142) \\ 
  & \\ 
 interaction\_term:n1000 & 92.186$^{***}$ \\ 
  & (0.460) \\ 

\hline 
\hline \\[-1.8ex]  
\end{tabular} 
\end{table}


\begin{comment}
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
  & \\ 
\hline \\[-1.8ex] 
Observations & 780,936 \\ 
R$^{2}$ & 0.998 \\ 
Adjusted R$^{2}$ & 0.998 \\ 
Residual Std. Error & 474.575 (df = 776673) \\ 
\end{comment}

==> graphics/did_employment.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Fr, Jan 05, 2024 - 16:42:16
\begin{table}[h] \centering 
  \caption{Fixed Effects Estimate} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & Employment \\ 
\hline \\[-1.8ex] 
 interaction\_term & 461.453$^{***}$ \\ 
  & (10.039) \\ 
\hline \\[-1.8ex] 
Observations & 1,859,178 \\ 
R$^{2}$ & 0.089 \\ 
Adjusted R$^{2}$ & 0.086 \\ 
Residual Std. Error & 6,240.190 (df = 1854009) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> graphics/did_wage.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Fr, Jan 05, 2024 - 14:54:38
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Annual Payroll}} \\ 
\cline{2-2} 
\\[-1.8ex] & ap \\ 
\hline \\[-1.8ex] 
 AI Exposure& $-$792.278$^{***}$ \\ 
  & (189.129) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 1,859,178 \\ 
R$^{2}$ & 0.054 \\ 
Adjusted R$^{2}$ & 0.051 \\ 
Residual Std. Error & 555,661.300 (df = 1854010) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> graphics/did_wage2.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Fr, Jan 05, 2024 - 16:42:14
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & ap \\ 
\hline \\[-1.8ex] 
 interaction\_term & 37,559.050$^{***}$ \\ 
  & (893.435) \\ 
  & \\ 
 post\_treatment & $-$250,350.200$^{***}$ \\ 
  & (5,700.140) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 1,859,178 \\ 
R$^{2}$ & 0.055 \\ 
Adjusted R$^{2}$ & 0.052 \\ 
Residual Std. Error & 555,372.600 (df = 1854009) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> graphics/did_wpemp.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Do, Jan 11, 2024 - 15:52:21
\begin{table}[!htbp] 
\centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & wage\_per\_emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 2.122$^{***}$ \\ 
  & (0.094) \\ 
\hline \\[-1.8ex] 
Observations & 1,271,079 \\ 
R$^{2}$ & 0.365 \\ 
Adjusted R$^{2}$ & 0.362 \\ 
Residual Std. Error & 32.218 (df = 1265924) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> graphics/na0_OV.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Di, Jan 16, 2024 - 10:26:38
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 72.763$^{***}$ \\ 
  & (0.889) \\ 
  & \\ 
 post\_treatment & $-$332.758$^{***}$ \\ 
  & (5.671) \\ 
  & \\ 
 n5\_9 & 15.799$^{***}$ \\ 
  & (0.048) \\ 
  & \\ 
 n10\_19 & 5.476$^{***}$ \\ 
  & (0.112) \\ 
  & \\ 
 n20\_49 & 31.081$^{***}$ \\ 
  & (0.099) \\ 
  & \\ 
 n50\_99 & 71.135$^{***}$ \\ 
  & (0.247) \\ 
  & \\ 
 n100\_249 & 154.992$^{***}$ \\ 
  & (0.312) \\ 
  & \\ 
 n250\_499 & 363.074$^{***}$ \\ 
  & (0.820) \\ 
  & \\ 
 n500\_999 & 544.907$^{***}$ \\ 
  & (1.651) \\ 
  & \\ 
 n1000 & 2,658.739$^{***}$ \\ 
  & (1.656) \\ 
  & \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table}

==> graphics/na0_emp.tex <==

\begin{comment}
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Do, Jan 11, 2024 - 17:25:48
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 67.584$^{***}$ \\ 
  & (0.902) \\ 
  & \\ 
 post\_treatment & $-$308.887$^{***}$ \\ 
  & (5.755) \\ 
  & \\ 
 n10\_19 & 37.384$^{***}$ \\ 
  & (0.053) \\ 
  & \\ 
 n20\_49 & 14.806$^{***}$ \\ 
  & (0.086) \\ 
  & \\ 
 n50\_99 & 71.518$^{***}$ \\ 
  & (0.250) \\ 
  & \\ 
 n100\_249 & 167.066$^{***}$ \\ 
  & (0.314) \\ 
  & \\ 
 n250\_499 & 362.605$^{***}$ \\ 
  & (0.834) \\ 
  & \\ 
 n500\_999 & 509.842$^{***}$ \\ 
  & (1.683) \\ 
  & \\ 
 n1000 & 1,973.766$^{***}$ \\ 
  & (3.459) \\ 
  & \\ 
 interaction\_term:n1000 & 108.869$^{***}$ \\ 
  & (0.479) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table}

\hline \\[-1.8ex] 
Observations & 1,859,178 \\ 
R$^{2}$ & 0.993 \\ 
Adjusted R$^{2}$ & 0.993 \\ 
Residual Std. Error & 559.927 (df = 1854001) \\ 
\end{comment}




% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Fr, Jan 12, 2024 - 11:45:16
\begin{table}[h] \centering 
  \caption{} 
  \label{}
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 65.986$^{***}$ \\ 
  & (0.877) \\ 
 n5\_9 & 15.472$^{***}$ \\ 
  & (0.048) \\ 
 n500\_999 & 509.666$^{***}$ \\ 
  & (1.637) \\ 
  & \\ 
 n1000 & 2,001.274$^{***}$ \\ 
  & (3.366) \\ 
  & \\ 
 interaction\_term:n1000 & 104.236$^{***}$ \\ 
  & (0.467) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> graphics/sd_emp.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: So, Jan 14, 2024 - 01:08:16
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp\_diff \\ 
\hline \\[-1.8ex] 
 AIGE & 15,177.450$^{***}$ \\ 
  & (1,400.573) \\ 
  & \\ 
 Constant & 36,909.400$^{***}$ \\ 
  & (1,791.813) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 3,126 \\ 
R$^{2}$ & 0.036 \\ 
Adjusted R$^{2}$ & 0.036 \\ 
Residual Std. Error & 98,842.090 (df = 3124) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

\begin{comment}
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Do, Jan 11, 2024 - 10:54:07
\begin{table}[!htbp] 
\centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 466.185$^{***}$ \\ 
  & (7.174) \\ 
  & \\ 
 Constant & 280.624$^{***}$ \\ 
  & (4.733) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 3,190,406 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 
\end{comment}

==> graphics/sd_emp_est.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: So, Jan 14, 2024 - 01:16:50
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & emp\_diff \\ 
\hline \\[-1.8ex] 
 AIGE & 14,825.410$^{***}$ \\ 
  & (1,392.664) \\ 
  & \\ 
 est & 73.781$^{***}$ \\ 
  & (11.459) \\ 
  & \\ 
 Constant & 34,900.570$^{***}$ \\ 
  & (1,807.452) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 3,126 \\ 
R$^{2}$ & 0.049 \\ 
Adjusted R$^{2}$ & 0.048 \\ 
Residual Std. Error & 98,208.210 (df = 3123) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> graphics/sd_wage.tex <==

\begin{table}[!htbp] \centering 
  \caption{First Difference Estimate on Wages per Employee} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & wage\_per\_emp\_diff \\ 
\hline \\[-1.8ex] 
 AIGE & 0.485$^{***}$ \\ 
  & (0.098) \\ 
\hline \\[-1.8ex] 
Observations & 3,126 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


\begin{comment}
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Do, Jan 11, 2024 - 10:54:05
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & wage\_per\_emp \\ 
\hline \\[-1.8ex] 
 interaction\_term & 4.929$^{***}$ \\ 
  & (0.038) \\ 
  & \\ 
 Constant & 36.483$^{***}$ \\ 
  & (0.046) \\ 
  & \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Do, Jan 11, 2024 - 10:54:07
%\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{comment}

==> graphics/sd_wage_est.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: So, Jan 14, 2024 - 01:16:50
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & wage\_per\_emp\_diff \\ 
\hline \\[-1.8ex] 
 AIGE & 0.477$^{***}$ \\ 
  & (0.098) \\ 
  & \\ 
 est & 0.002$^{**}$ \\ 
  & (0.001) \\ 
  & \\ 
 Constant & 13.072$^{***}$ \\ 
  & (0.127) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 3,126 \\ 
R$^{2}$ & 0.009 \\ 
Adjusted R$^{2}$ & 0.009 \\ 
Residual Std. Error & 6.915 (df = 3123) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 
